ResNCT: A Deep Learning Model for the Synthesis of Nephrographic Phase Images in CT Urography

Purpose: To develop and evaluate a transformer-based deep learning model for the synthesis of nephrographic phase images in CT urography (CTU) examinations from the unenhanced and urographic phases. Materials and Methods: This retrospective study was approved by the local Institutional Review Board. A dataset of 119 patients (mean $\pm$ SD age, 65 $\pm$ 12 years; 75/44 males/females) with three-phase CT urography studies was curated for deep learning model development. The three phases for each patient were aligned with an affine registration algorithm. A custom model, coined Residual transformer model for Nephrographic phase CT image synthesis (ResNCT), was developed and implemented with paired inputs of non-contrast and urographic sets of images trained to produce the nephrographic phase images, that were compared with the corresponding ground truth nephrographic phase images. The synthesized images were evaluated with multiple performance metrics, including peak signal to noise ratio (PSNR), structural similarity index (SSIM), normalized cross correlation coefficient (NCC), mean absolute error (MAE), and root mean squared error (RMSE). Results: The ResNCT model successfully generated synthetic nephrographic images from non-contrast and urographic image inputs. With respect to ground truth nephrographic phase images, the images synthesized by the model achieved high PSNR (27.8 $\pm$ 2.7 dB), SSIM (0.88 $\pm$ 0.05), and NCC (0.98 $\pm$ 0.02), and low MAE (0.02 $\pm$ 0.005) and RMSE (0.042 $\pm$ 0.016). Conclusion: The ResNCT model synthesized nephrographic phase CT images with high similarity to ground truth images. The ResNCT model provides a means of eliminating the acquisition of the nephrographic phase with a resultant 33% reduction in radiation dose for CTU examinations.

==> references.tex <==
@article{silverman2009current,
  title={What is the current role of CT urography and MR urography in the evaluation of the urinary tract?},
  author={Silverman, Stuart G and Leyendecker, John R and Amis Jr, E Stephen},
  journal={Radiology},
  volume={250},
  number={2},
  pages={309--323},
  year={2009},
  publisher={Radiological Society of North America}
}

@article{nawfel2004patient,
  title={Patient radiation dose at CT urography and conventional urography},
  author={Nawfel, Richard D and Judy, Philip F and Schleipman, A Robert and Silverman, Stuart G},
  journal={Radiology},
  volume={232},
  number={1},
  pages={126--132},
  year={2004},
  publisher={Radiological Society of North America}
}

@article{cheng2019ct,
  title={CT urography: how to optimize the technique},
  author={Cheng, Karen and Cassidy, Fiona and Aganovic, Lejla and Taddonio, Michael and Vahdat, Noushin},
  journal={Abdominal Radiology},
  volume={44},
  pages={3786--3799},
  year={2019},
  publisher={Springer}
}

@article{potenta2015ct,
  title={CT urography for evaluation of the ureter},
  author={Potenta, Scott E and D'Agostino, Robert and Sternberg, Kevan M and Tatsumi, Kanayo and Perusse, Karina},
  journal={Radiographics},
  volume={35},
  number={3},
  pages={709--726},
  year={2015},
  publisher={Radiological Society of North America}
}

@article{chow2007split,
  title={Split-bolus MDCT urography with synchronous nephrographic and excretory phase enhancement},
  author={Chow, Lawrence C and Kwan, Sharon W and Olcott, Eric W and Sommer, Graham},
  journal={American Journal of Roentgenology},
  volume={189},
  number={2},
  pages={314--322},
  year={2007},
  publisher={Am Roentgen Ray Society}
}

@article{raman2017upper,
  title={Upper and lower tract urothelial imaging using computed tomography urography},
  author={Raman, Siva P and Fishman, Elliot K},
  journal={Radiologic Clinics},
  volume={55},
  number={2},
  pages={225--241},
  year={2017},
  publisher={Elsevier}
}

@article{morrison2021split,
  title={Split vs. Single Bolus CT Urography: Comparison of scan time, image quality and radiation dose},
  author={Morrison, Nicole and Bryden, Sherrie and Costa, Andreu F},
  journal={Tomography},
  volume={7},
  number={2},
  pages={210--218},
  year={2021},
  publisher={MDPI}
}

@article{dillman2007comparison,
  title={Comparison of urinary tract distension and opacification using single-bolus 3-phase vs split-bolus 2-phase multidetector row CT urography},
  author={Dillman, Jonathan R and Caoili, Elaine M and Cohan, Richard H and Ellis, James H and Francis, Isaac R and Nan, Bin and Zhang, Yong},
  journal={Journal of computer assisted tomography},
  volume={31},
  number={5},
  pages={750--757},
  year={2007},
  publisher={LWW}
}

@inproceedings{pasternak2012clinical,
  title={Clinical pharmacology, uses, and adverse reactions of iodinated contrast agents: a primer for the non-radiologist},
  author={Pasternak, Jeffrey J and Williamson, Eric E},
  booktitle={Mayo Clinic Proceedings},
  volume={87},
  pages={390--402},
  year={2012},
  organization={Elsevier}
}

@article{dalmaz2022resvit,
  title={ResViT: residual vision transformers for multimodal medical image synthesis},
  author={Dalmaz, Onat and Yurt, Mahmut and {\c{C}}ukur, Tolga},
  journal={IEEE Transactions on Medical Imaging},
  volume={41},
  number={10},
  pages={2598--2614},
  year={2022},
  publisher={IEEE}
}

@article{schwartz1994kidney,
  title={Kidney mobility during respiration},
  author={Schwartz, Laurent H and Richaud, Jocelyne and Buffat, Laurent and Touboul, Emmanuel and Schlienger, Michel},
  journal={Radiotherapy and Oncology},
  volume={32},
  number={1},
  pages={84--86},
  year={1994},
  publisher={Elsevier}
}

@inproceedings{isola2017image,
  title={Image-to-image translation with conditional adversarial networks},
  author={Isola, Phillip and Zhu, Jun-Yan and Zhou, Tinghui and Efros, Alexei A},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1125--1134},
  year={2017}
}

@article{saxena2021comparison,
  title={Comparison and analysis of image-to-image generative adversarial networks: a survey},
  author={Saxena, Sagar and Teli, Mohammad Nayeem},
  journal={arXiv preprint arXiv:2112.12625},
  year={2021}
}

@inproceedings{ye2013modality,
  title={Modality propagation: coherent synthesis of subject-specific scans with data-driven regularization},
  author={Ye, Dong Hye and Zikic, Darko and Glocker, Ben and Criminisi, Antonio and Konukoglu, Ender},
  booktitle={Medical Image Computing and Computer-Assisted Intervention--MICCAI 2013: 16th International Conference, Nagoya, Japan, September 22-26, 2013, Proceedings, Part I 16},
  pages={606--613},
  year={2013},
  organization={Springer}
}

@inproceedings{huo2018adversarial,
  title={Adversarial synthesis learning enables segmentation without target modality ground truth},
  author={Huo, Yuankai and Xu, Zhoubing and Bao, Shunxing and Assad, Albert and Abramson, Richard G and Landman, Bennett A},
  booktitle={2018 IEEE 15th international symposium on biomedical imaging (ISBI 2018)},
  pages={1217--1220},
  year={2018},
  organization={IEEE}
}

@article{huang2017cross,
  title={Cross-modality image synthesis via weakly coupled and geometry co-regularized joint dictionary learning},
  author={Huang, Yawen and Shao, Ling and Frangi, Alejandro F},
  journal={IEEE transactions on medical imaging},
  volume={37},
  number={3},
  pages={815--827},
  year={2017},
  publisher={IEEE}
}

@article{yi2019generative,
  title={Generative adversarial network in medical imaging: A review},
  author={Yi, Xin and Walia, Ekta and Babyn, Paul},
  journal={Medical image analysis},
  volume={58},
  pages={101552},
  year={2019},
  publisher={Elsevier}
}

@article{litjens2017survey,
  title={A survey on deep learning in medical image analysis},
  author={Litjens, Geert and Kooi, Thijs and Bejnordi, Babak Ehteshami and Setio, Arnaud Arindra Adiyoso and Ciompi, Francesco and Ghafoorian, Mohsen and Van Der Laak, Jeroen Awm and Van Ginneken, Bram and S{\'a}nchez, Clara I},
  journal={Medical image analysis},
  volume={42},
  pages={60--88},
  year={2017},
  publisher={Elsevier}
}

@article{choi2021generating,
  title={Generating synthetic contrast enhancement from non-contrast chest computed tomography using a generative adversarial network},
  author={Choi, Jae Won and Cho, Yeon Jin and Ha, Ji Young and Lee, Seul Bi and Lee, Seunghyun and Choi, Young Hun and Cheon, Jung-Eun and Kim, Woo Sun},
  journal={Scientific reports},
  volume={11},
  number={1},
  pages={20403},
  year={2021},
  publisher={Nature Publishing Group UK London}
}

@article{ristea2023cytran,
  title={CyTran: a cycle-consistent transformer with multi-level consistency for non-contrast to contrast CT translation},
  author={Ristea, Nicolae-C{\u{a}}t{\u{a}}lin and Miron, Andreea-Iuliana and Savencu, Olivian and Georgescu, Mariana-Iuliana and Verga, Nicolae and Khan, Fahad Shahbaz and Ionescu, Radu Tudor},
  journal={Neurocomputing},
  volume={538},
  pages={126211},
  year={2023},
  publisher={Elsevier}
}

@article{dayarathna2023deep,
  title={Deep learning based synthesis of MRI, CT and PET: Review and analysis},
  author={Dayarathna, Sanuwani and Islam, Kh Tohidul and Uribe, Sergio and Yang, Guang and Hayat, Munawar and Chen, Zhaolin},
  journal={Medical Image Analysis},
  pages={103046},
  year={2023},
  publisher={Elsevier}
}

